Striking the Right Balance: Recall Loss for Semantic Segmentation

Class imbalance is a fundamental problem in computer vision applications such as semantic segmentation. Specifically, uneven class distributions in a training dataset often result in unsatisfactory performance on under-represented classes. Many works have proposed to weight the standard cross entropy loss function with pre-computed weights based on class statistics, such as the number of samples and class margins. There are two major drawbacks to these methods: 1) constantly up-weighting minority classes can introduce excessive false positives in semantic segmentation; 2) a minority class is not necessarily a hard class. The consequence is low precision due to excessive false positives. In this regard, we propose a hard-class mining loss by reshaping the vanilla cross entropy loss such that it weights the loss for each class dynamically based on instantaneous recall performance. We show that the novel recall loss changes gradually between the standard cross entropy loss and the inverse frequency weighted loss. Recall loss also leads to improved mean accuracy while offering competitive mean Intersection over Union (IoU) performance. On Synthia dataset, recall loss achieves $9\%$ relative improvement on mean accuracy with competitive mean IoU using DeepLab-ResNet18 compared to the cross entropy loss. Code available at https://github.com/PotatoTian/recall-semseg.

==> figure/synthia.tex <==
\begin{figure*}
\centering
     \includegraphics[width=0.9\textwidth]{figure/synthia.png}
     \caption{Mean accuracy vs.  mean intersection over union (IOU) on Synthia dataset with Deeplab - ResNet18 (left)/-ResNet101 (right). Recall loss improves mean accuracy while maintaining a competitive mean IoU.}
     \label{fig:synthia_overall}
\end{figure*}




==> table/synthia.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|cccccccc|cccccccc} 
    \toprule
     &\multicolumn{8}{c}{ResNet18}& \multicolumn{8}{c}{ResNet101}\\
     \midrule
     &CE& SoftIOU& Lovasz& OHEM & Weighted & Balanced & Focal& Recall &CE& SoftIOU& Lovasz& OHEM & Weighted & Balanced & Focal& Recall\\
     \midrule
    mIoU & 80.26 & 81.07 & 78.62 & 64.36 & 76.04 & 74.19 & 80.71 & 81.45
        & 83.73 & \textbf{84.69} & 71.59 & 65.92 & 75.27 & 76.25 & 82.82 & 83.21 \\
    mACC & 84.68 & 89.11 & 88.59 & 78.42 & 96.26 & 96.49 & 85.77 & 92.36
        & 88.05 & 91.77 & 92.75 & 83.76 & 96.68 & 97.47  & 87.42 & 95.06\\
    \midrule
    mIoU* & 94.62 & 93.86 & 93.92 & 84.98 &	93.37 &	93.06 &	94.48 &	94.35
        & 94.77 & 93.83 &	92.62 &	83.48 &	91.90 &	92.58 &	94.20 &	94.18\\
    mACC* & 97.16 &	96.76 & 96.79 &	90.07 &	97.06 &	96.87 & 97.24 &	97.15
        & 97.23 &	96.88 &	96.16 &	93.57 &	97.25 &	97.53 &	96.86 &	97.75\\
    \midrule
    mIoU$\dag$ & 56.52  & 59.77 & 52.76 & 30.79 & 47.50 & 43.41 & 58.09 & 60.28
        & 63.8 & 68.26 & 48.06 & 34.32 & 45.33 & 46.85 & 62.32 & 63.45\\
    mACC$\dag$ & 63.54 & 76.18 & 74.60 & 57.68 & 94.68 & 95.60 & 66.65 & 84.09
        & 71.53 & 82.56 & 86.62 & 66.10 & 95.66 & 97.36 & 70.43 & 90.20\\
    \bottomrule
    \end{tabular}}
     \caption{\textbf{DeepLab ResNet18 abd101 performance on Synthia-Summer}. * denotes average performance of higher performance classes. $\dag$ denotes performance across classes of IoU lower than $80$ with CE loss.}
    \label{tab:synthia}
\end{table*}
